Investigation of Algorithms for Highly Nonlinear Model Fitting on Big Datasets

This thesis investigates algorithms regarding their applicability for highly nonlinear model fitting on big datasets. Various mathematical methods are presented with which a model fit using the least squares criterion is possible. Special requirements regarding the processing of large data sets as a basis for such a model fit are discussed. The specific example of the search for gravitational wave signals in simulated data of the ESA satellite mission Gaia is used to demonstrate how a model fit is possible, even with complex models and large amount of data. For this purpose, a highly parallel prototype of a future search software is implemented. The resulting prototype uses a hybrid algorithm which utilizes a linear search, an evolutionary algorithm and a classical iterative Gauss-Newton fit. The performance and behavior of its components are investigated in detail. With the help of software presented in this work it has been possible for the first time to detect gravitational wave signals in simulated astrometric data, and to determine their parameters. Furthermore, it can be concluded from the runtime behavior of the software that such a search is also possible in real data of the Gaia mission.

==> content/math-chapter_begin-nonlinear.tex <==
To to somehow classify different approaches in nonlinear parameter estimation, in the following chapters, three different types of model fitting are discussed:
\begin{itemize}
 \item Linear model fitting
 \item Nonlinear model fitting
 \item Highly (or strong) nonlinear fitting
\end{itemize}
Whilst the difference between linear and nonlinear fitting is strict. The differentiation between the last two is somewhat arbitrary. A linear model function is a function $f\left( x; a_1...a_M \right)$ with $M$ free parameters in a general linear combination, which can be expressed as a harmonic series:

\begin{equation}
\label{eq:least-squares-lin-model}
f\left( x;a_1...a_M \right) = \sum_{k=1}^{M}a_k X_k(x)
\end{equation}

With $X_k(x)$ are arbitrary fixed functions, called the basic functions, which even can be nonlinear. The linearity or nonlinearity of a model only depends on the parameters $a_k$.

\bigskip

On the other hand, a nonlinear model function, can not be expressed as a linear combination of functions. One example is $f(x;a_0)=\sin a_o x$, where $a_0$ is clearly nonlinear. In general, every parameter, which does not cancel out in a partial derivative is nonlinear. \correctme{partial derivative better/clearer}

\bigskip

The term ``highly nonlinear'' problem is somewhat arbitrary, but can be described by some main features. The first one is noise which dominates the data to fit. This leads to a almost chaotic behavior of the sum of squared residues in the fit. Another feature of highly nonlinear problems is that the parameter space can not be probed in reasonable time. In almost every case heuristic optimization algorithms have to be used to achieve a (more or less) optimal solution.

\section{Nonlinear Least Square Fitting}
In general least square fitting is process which tries to minimize the residues between a model function and observations. One residue $r_i$ is defined as
\begin{equation}
 \label{eq:least-squares-r}
r_i = y_i - f\left( x_i;\mb{p} \right)
\end{equation}
Were $f$ is the model function with the parameter vector $\mb{p}$, and $y_i$ are the observed values for a specific $x_i$. The sum of the squared residues is defined as 
\begin{equation}
 \label{eq:least-squares-S}
S = \sum_i^N r_i^2~\text{.}
\end{equation}
The method of least squares tries to minimize $S$, which is the case when the gradient of the squared residues becomes zero:
\begin{equation}
 \label{eq:least-squares-partial}
\dfrac{\partial S}{\partial p_j} = 2\sum_i^N r_i \dfrac{\partial r_i}{\partial p_j} = 0 ~~~~ (j=0,..,M)~\text{.}
\end{equation}
Inserting \ref{eq:least-squares-r} into \ref{eq:least-squares-partial} yields
\begin{equation}
 \label{eq:least-squares-finpart}
\dfrac{\partial S}{\partial p_j} = -2\sum_i^N r_i \dfrac{\partial f\left( x_i;\mb{p} \right)}{\partial p_j} = 0 ~~~~ (j=0,..,M)~\text{.}
\end{equation}
Which can be expressed in the following matrix equations
\begin{align}
 \label{eq-least-squares-mateq}
\mb{A}^T\mb{b} &= \mb{A}^T\mb{A}\mb{\delta}\\
A_{ij} &= \dfrac{\partial f\left( x_i;\mb{p} \right)}{\partial p_j}\\
b_{i}  &= y_i - f\left( x_i;\mb{p} \right)
\end{align}
By solving for $\mb{\delta}$ one get the refinement for the parameters $\mb{p}$. The result can be applied to the starting parameters and the matrix equations can be solved iteratively until the refinement is below a certain $\varepsilon$.

\section{Linear Least Square Fitting}
In case of a linear model (like described in \ref{eq:least-squares-lin-model}), the design equations simplify since,
\begin{equation}
 \label{eq:lin-model-partial}
\dfrac{\partial f\left( x_i;\mb{p} \right)}{\partial p_j} = X_j\left(x_i\right)~\text{.}
\end{equation}
So the matrix equations becoming
\begin{align}
 \label{eq-least-squares-mateqlin}
\mb{A}^T\mb{b} &= \mb{A}^T\mb{A}\mb{p}\\
A_{ij} &= X_j\\
b_{i}  &= y_i
\end{align}
Solving for $\mb{p}$ directly yields the result parameters. Also note, that no starting values are necessary, since the design matrix $\mb{A}$ only contain the base functions at the points $x_i$.

\section{Highly Nonlinear Model Fitting}
An example might be is the best way to show the problems introduced by a high amount of noise and a growing parameter space. Just assume we want to fit a multi dimensional sine function to some data. Our model is

\begin{equation}
 \label{eq:simple-sine-model}
y(\mb{x};t) = s(\mb{x};t) + n(t) = \sum_{i=1}^N \left(  A_i \sin \left(\omega_i x \right) \right) + n(t)
\end{equation}

where $A_i$ are the amplitudes, $\omega_i$ is the frequencies and $n(t)$ is some noise. As one can see $A_i$ are linear parameters, while $\omega_i$ are nonlinear parameters.
Using the standard Mathematica routines for nonlinear parameter estimations, one can clearly see how the complexity grows with additional parameters (i.e. dimensions) and accuracy drops with growing noise. Table~\ref{tab:mathematica_simple_noise} shows the result of some experiment, regarding this issue.

\begin{table}[H]
\centering
\begin{tabular}{lll} \toprule
Number of Dimensions		& Noise Factor		& Runtime \\ \midrule
1							& 0					& \\
1							& 1					& \\
1							& 10				& \\
1							& 100				& \\
3							& 0					& \\
3							& 1					& \\
3							& 10				& \\
3							& 100				& \\
6							& 0					& \\
6							& 1					& \\
6							& 10				& \\
6							& 100				& \\
12							& 0					& \\
12							& 1					& \\
12							& 10				& \\
12							& 100				& \\ \bottomrule
\end{tabular}
\caption[Simple experiment for highly nonlinear parameter estimation in Mathematica]{A simple experiments shows how difficult it becomes to fit a high dimensional nonlinear model with noisy data. The experiment was conducted on an standard notebook using Mathematica 9.0.1, using 5000 randomly sampled data points. Gaussian noise was added and multiplied by the noise factor. \textborn~marks fits where no result could be found, or was completely off.\label{tab:mathematica_simple_noise}}
\end{table}




% In general, least square fitting is the minimization of
% \begin{equation}
% \label{eq:least-squares}
% \sum_{i=1}^{N}\left( y_i - y\left( x_i;\mb{a} \right) \right)^2
% \end{equation}
% where $(y_i,x_i)$ with $i=1,...,N$ are $N$ measured or otherwise obtained data points. And $\mb{a} = \left[ a_1, ..., a_M \right]^T $ is a set of $M$ linear parameters. Let $\mb{G}$ be a $N\times M$ matrix which contains the result of the basis functions $X_k(x_i)$ (see equation \ref{eq:least-squares-lin-model}) for all $i=1...N$ data points. The construction of $\mb{G}$ is as follows.
% 
% \begin{equation}
%  \label{eq:design-matrix}
% G_{ij}=\dfrac{X_j(x_i)}{\sigma_i}
% \end{equation}
% 
% Furthermore, let $\mb{d}$ be a vector of data values at the positions $x_i$, with the standard deviation $\sigma_i$ for each point taken into account. If the standard deviations for a data point $i$ is not know, set all $\sigma_i = 1$ as proposed in (\cite{NRC-1992} p. 671)
% 
% \begin{equation}
%  \label{eq:data-vector-b}
% d_i = \dfrac{y_i}{\sigma_i}
% \end{equation}
% 
% The solution for the least square problem is then given trough matrix $\mb{A}$
% \begin{equation}
%  \label{eq:solution-least-square-normal-eq}
% \mb{A} = \left( \mb{G}^T \mb{G} \right)^{-1} \mb{G^T} \mb{d}
% \end{equation}
% 
% The inverse matrix $\mb{C} = \left( \mb{G}^T \mb{G} \right)^{-1}$ is called the covariance matrix, the elements $C_{jj}$ are the fitted squared standard deviations of the parameters $a_j$. Off-diagonal elements are the covariances of the parameters respectively.
% 
% \bigskip
% 
% As described in \cite{NRC-1992}, the method described above is suitable for most problems but can lead to (near) singular normal equations. An alternative approach is the solution using singular value decomposition (SVD). Which, in fact, most libraries which provide least square fitting routines employ.

